ALFRED: A Benchmark for Interpreting Grounded Instructions for Everyday Tasks

We present ALFRED (Action Learning From Realistic Environments and Directives), a benchmark for learning a mapping from natural language instructions and egocentric vision to sequences of actions for household tasks. ALFRED includes long, compositional tasks with non-reversible state changes to shrink the gap between research benchmarks and real-world applications. ALFRED consists of expert demonstrations in interactive visual environments for 25k natural language directives. These directives contain both high-level goals like "Rinse off a mug and place it in the coffee maker." and low-level language instructions like "Walk to the coffee maker on the right." ALFRED tasks are more complex in terms of sequence length, action space, and language than existing vision-and-language task datasets. We show that a baseline model based on recent embodied vision-and-language tasks performs poorly on ALFRED, suggesting that there is significant room for developing innovative grounded visual language understanding models with this benchmark.

==> tables/assist_tasks_table.tex <==
\begin{table}
\centering
\begin{small}
\begin{tabular}{@{}l@{\hspace{8pt}}acacac@{}}
           & \multicolumn{6}{c}{Sub-Goal Ablations - \textbf{Validation}} \\
           & \mcc{2}{\basemodels{Vision-only}} & \mcc{2}{\basemodels{Seq2Seq}} & \multicolumn{2}{@{}c@{}}{\basemodels{Seq2Seq+PM}}    \\
Sub-Goal   & \splits{Seen}   &\splits{Unseen} & \splits{Seen} & \splits{Unseen} & \splits{Seen} & \splits{Unseen} \\
\toprule
Goto       & 27.6     & 17.0    &    49.0    & 20.7     & \B{50.8}   & \B{21.6} \\ 
Pickup     & 22.4     &  9.3    &    31.8    & 20.2     & \B{32.5}   & \B{20.9} \\ 
Put        & 70.8     & 31.0    &    80.0    & \B{50.8} & \B{81.4}   &    45.7  \\ 
Cool       & \B{88.8} & 74.9    &    87.1    & \B{94.3} &    88.1    &    92.3 \\  
Heat       & \B{86.8} & 85.7    &    84.9    & 88.2     &    84.9    & \B{89.3} \\ 
Clean      & 65.2     & 16.8    &    82.0    & 29.9     & \B{83.8}   & \B{56.0} \\ 
Slice      & 22.6     & 14.1    &    27.3    & 18.8     & \B{31.6}   & \B{25.6} \\ 
Toggle     & 90.4     &  5.0    &    96.8    & 53.7     & \B{100.0}  & \B{57.9} \\  
\midrule                             
Average    & 59.4     &  32.5   & 67.3    & 47.3    & \B{68.7}  & \B{51.4}  \\ 
\bottomrule
\end{tabular}
\end{small}
\caption{\textbf{Evaluations by path weighted sub-goal success.}
The highest values per fold and task are shown in \B{blue}.
We note that the \basemodels{Language-only} model achieves less than 2\% on all sub-goals.
See supplemental material for more.}
\label{tab:subtask_abblations}
\end{table}


==> tables/step_by_step.tex <==
\begin{table}
\centering
\begin{small}
\begin{tabular}{@{}laacc@{}}
             %& \multicolumn{4}{c}{\textbf{Validation}}\\
             & \multicolumn{2}{b}{\splits{Seen}} & \multicolumn{2}{c}{\splits{Unseen}}\\
Model        & Task & Goal-Cond & Task & Goal-Cond \\
\toprule  
All Inputs   & \B{3.0} (\B{1.2}) & \B{10.0} (\B{6.0}) & 0.1 (0.0) & 6.9 (4.9) \\
Step-by-Step &    2.8 (1.6) &  9.1 (6.8) & 0.1 (0.0) & 7.7 (5.4) \\
\hspace{1em} 
  w/ History &    2.1 (1.4) &  9.2 (6.9) & \B{0.5} (\B{0.3}) & \B{7.8} (\B{5.8}) \\
\bottomrule
\end{tabular}
\end{small}
\label{tab:step_by_step_abblations}
\caption{Oracle step-by-step evaluation}
\end{table}
